Multimodal Visual-haptic pose estimation in the presence of transient occlusion

Human-robot collaboration requires the establishment of methods to guarantee the safety of participating operators. A necessary part of this process is ensuring reliable human pose estimation. Established vision-based modalities encounter problems when under conditions of occlusion. This article describes the combination of two perception modalities for pose estimation in environments containing such transient occlusion. We first introduce a vision-based pose estimation method, based on a deep Predictive Coding (PC) model featuring robustness to partial occlusion. Next, capacitive sensing hardware capable of detecting various objects is introduced. The sensor is compact enough to be mounted on the exterior of any given robotic system. The technology is particularly well-suited to detection of capacitive material, such as living tissue. Pose estimation from the two individual sensing modalities is combined using a modified Luenberger observer model. We demonstrate that the results offer better performance than either sensor alone. The efficacy of the system is demonstrated on an environment containing a robot arm and a human, showing the ability to estimate the pose of a human forearm under varying levels of occlusion.

==> sections/sensor_design.tex <==
%\section{Sensor Design} \label{sec:sensor_design}

A simplified schematic of a single capacitive sensor is shown in Fig. \ref{fig:efield_schematic}. We propose a design based on the one introduced in \cite{smith1999electric}. It consists of two subcircuits, one to generate the electric field (left side of Fig. \ref{fig:efield_schematic}), the other to measure this field (right). 
Field generation is performed via an inductor-capacitor circuit (LC tank). A metal plate (the \textit{excitation electrode}) is attached in parallel to the capacitor. Applying an Alternating Current (AC) after frequency matching the resonance frequency of the LC tank generates a high-voltage AC at the \textit{excitation electrode}, creating an electric field in its surroundings.
The field is measured by means of a second metal plate, the \textit{sensing electrode}. The measured signal is amplified by an operational amplifier.
Ground plates are included to help influence the field's shape, shielding the sensors from interference generated by neighboring circuits. When mounted on a robotic arm, the plates also help mitigate measurement distortions caused by the electric field generated by the robot's actuators.

As the presence of nearby objects alter the electric field in proximity to the electrodes, the measured voltage at the sensing electrode changes accordingly. In particular, when an object with a sufficient dielectric constant $\epsilon_{\text r}$ is introduced in proximity to the sensor, its presence alters the field's shape, generating a measurable change in the sensing electrode, thus ensuring detection.
As previously mentioned, human tissue possesses a high $\epsilon_{\text r}$, facilitating its perception by the proposed setup. 

\begin{figure}
	\centering
	\def\svgwidth{1.05\columnwidth}
	%\hspace{-1.5em}%
	\input{images/hardware_board.pdf_tex}%
	\caption{Capacitive sensor signal processing board, with individual sections marked.}
	\vspace{1em}
	\label{fig:measure_board}
\end{figure}

\begin{figure}
	\centering
	\begin{subfigure}{0.49\columnwidth}%
		\centering
		\def\svgwidth{\textwidth}
		\includegraphics[width=\textwidth,height=102px]{images/sensor_cropped_compressed.png}
		%\caption{Second subfigure.}
		%\label{fig:five_sensor_board}
	\end{subfigure}%
	\hfill%
	\begin{subfigure}{0.49\columnwidth}%
		\centering
		\def\svgwidth{1.0\textwidth}
		\input{images/sensor_5_circular_board.pdf_tex}
		%\caption{Firts subfigure.}
		%\label{fig:measure_board}
	\end{subfigure}%
	\caption{Setup combining the signal processing with the electrode board (left) and diagram (right) consisting of one excitation electrode (middle, dark red ring) and five measurement electrodes (\textbf{c}enter, \textbf{l}eft, \textbf{r}ight, \textbf{t}op, \textbf{b}ottom).}
	%\vspace{-1.5em}
	\label{fig:electrode_board}
\end{figure}

We propose a simple capacitive sensor design featuring minimal components. We developed a custom circuit supporting both signal generation and processing, shown in Fig. \ref{fig:measure_board}. The board can interface with multiple sensing and emission electrodes simultaneously. Its schematics can be found \href{https://github.com/Mike2208/active_electric_perception}{\tt {\small here}}. It is composed of two inductor-capacitor tank circuits (labelled {\tt LCT1} and {\tt LCT2} in Fig. \ref{fig:measure_board}), two operational amplifiers ({\tt AMP}), a central microcontroller ({\tt MCU}), and a Universal Asynchronous Receiver-Transmitter to Universal Serial Bus (UART-to-USB) communication interface ({\tt COMM}).
The {\tt LCT} circuits offer a compact way of generating high-voltage sine waves from a low-voltage alternating current source. A simplified schematic is provided in Fig. \ref{fig:efield_schematic} (left side). We use the integrated Pulse Width Modulators (PWM) of the {\tt MCU} to provide the requisite input. The resulting high voltage AC is fed into the capacitive sensor's excitation electrode. Note that while the resulting voltage is in the range of 20V, the energy within the excitation circuit is low enough to guarantee the safety of nearby participants even when directly in contact with the electrodes. Generally, a high-frequency field is desirable, as it is less susceptible to noise (see \cite{smith1999electric}). However, high frequencies also require faster signal processing methods, which in turn rely on larger, more complex and costly hardware. Our circuit relies on a single microcontroller, allowing development of a small, compact board. However, the simplified design also limits the maximum signal frequency. For our specific implementation, we determined that the MCU's PWMs are sufficient for an LC circuit with a resonance frequency of approximately $100\text{kHz}$ (with $L=25\text{mH}$, $C=1\text{nF}$).
The {\tt AMP} circuits are connected to the sensing electrodes, applying a constant gain to the voltage measured at each electrode. The amplified signal is fed to the Analog-Digital Converter (ADC) of the microcontroller. Each {\tt AMP} circuit can be connected to 4 electrodes simultaneously allowing the board to process 8 sensor measurements in total.
The {\tt MCU}, based on the PIC32MK by Microchip (\cite{pic32mk}), is used for signal generation and processing. Adjusting the PWM signal it generates can allow to drive a range of different {\tt LCT} designs beyond the setup considered here. The integrated ADC module supports sampling rates up to 20MSamples/s. This, combined with its 6 unique ADC modules allows us to connect and process signals from multiple sensing electrodes simultaneously. Our hardware is configured to collect measures from up to 18 individual electrodes, with each ADC alternating between 3 inputs.
Finally, the {\tt COMM} provides a communication link between the {\tt MCU} and a connected Personal Computer (PC) through a UART interface.

The firmware installed on the {\tt MCU} along with the required PC software can be found \href{https://github.com/Mike2208/active_electric_perception}{\tt {\small here}}. The microcontroller is programmed to generate a high-voltage AC signal at an adjustable frequency for the emitting electrode and to process incoming signals measured on the sensing electrodes.
The following provides a brief overview of signal generation and processing. By adjusting the PWM to output a square wave at a frequency of $f_{\text e}$ Hz, the system generates an excitation signal at the emission electrode with the same frequency. Measurements are taken at a sampling frequency of $f_{\text s} = 4f_{\text e}$ Hz. In plain words, we measure four samples per PWM cycle.
The measured voltage at the sensing electrode is noted as $v_{\text{s}k}, k \in \mathds{N}$ at time instant $t=k/f_{\text s}$, in V.
Note that the {\tt MCU} does not provide the computational power required to analyze the gathered measures. Instead, measures are sent to a PC for signal processing. 
As we are generating a sine wave at the emission electrode with a frequency of $f_{\text e}$, the measures at the sensing electrode will follow a similar pattern. In practice, this measure materializes in the form of a sine wave signal at the sensing electrode, which may be reconstructed from samples using Fourier series decomposition. Note that the requisite Nyquist criteria is satisfied, as $f_{\text s} \geqslant 2f_{\text e}$. We compute the signal amplitude as $v_{\text{m}n} = \sqrt{s_{n}^2 + c_{n}^2}$, where

\begin{equation}
	s_{n} = \sum_{k=n}^{n+3} v_{\text{s}k} \sin \left( 2\pi f_{\text e} k \right), \quad c_{n} = \sum_{k=n}^{n+3} v_{\text{s}k} \cos \left( 2\pi f_{\text e} k \right), \nonumber
\end{equation}%
in which $s_{n}, c_{n}\in \mathds{R}$ are the Fourier series coefficients of the sampled measures for the excitation frequency $f_{\text e}$ in V, and $v_{\text{m}n} \in \mathds{R}^+$ is the amplitude of the measured voltage at the sensing electrode in V.
Subsequent noise reduction is performed by averaging over multiple consecutive measures $v_{\text{m}n}$. Assuming that $v_{\text{m}n}$ changes slowly between samples, the Signal-to-Noise Ratio (SNR) is improved by a factor of $\sqrt{i}$, where $i$ is the number of averaged sequential samples $v_{\text{m}n}$ (as described in \cite{hassan2010reducing}). 
As our sampling time is in the order of $t = 0.01 \text{ms}$ and human movements have a time constant in the order of seconds, the value of $v_{\text{m}n}$ will remain near constant over a range of $i=100$ measures (time window of 1 ms), improving sensor SNR by a factor of 10. Experimental results in section \ref{sec:experimental_results} confirm this assumption.
We define a continuous time-counterpart $v_\text{m}(t), t\geqslant0$ (in V) to $v_{\text{m}n}$, with $v_\text{m}(t) \equiv v_{\text{m}k}, \quad t \in \left[ (k-1)/f_\text{e}, k/f_\text{e} \right), k \in \mathds{N}$.
%
%\begin{equation}
%v_\text{m}(t) = v_{\text{m}k}, \quad t \in \left[ (k-1)/f_\text{e}, k/f_\text{e} \right), k \in \mathds{N}.
%\end{equation}%
%
The value of $v_{\text m}(t)$ changes when the electric field is altered by the introduction of an object into the sensor's range. In Section \ref{sec:experimental_results}, we characterize how the proximity to  various objects affects $v_{\text m}(t)$.

In addition to object detection, $v_{\text m}(t)$ is also used to help calibrate $f_{\text e}$. This is necessary as the shape of the excitation electrode impacts the effective capacitance in the LC circuit described above, thereby altering the value of its resonance frequency.
The value of $f_{\text e}$ is adapted using gradient descent.
This calibration is only required when the setup is changed significantly, e.g. when the processing board is first powered on, or when electrode shapes are meaningfully altered. The current hardware is able to set $f_{\text e}$ to values in the range of 50kHz to 120kHz.

%\begin{figure*}
%	\centering
%	\begin{subfigure}{\columnwidth}
%		\centering
%		\def\svgwidth{\columnwidth}
%		\input{images/sensor_size_compare.pdf_tex}
%		\caption{Sensor sensitivity to a human hand depending on sensor area. The larger the area, the higher the relative voltage change when a hand gets near.}
%	\end{subfigure}%
%	\hfill%
%	\begin{subfigure}{\columnwidth}
%		\centering
%		\def\svgwidth{\columnwidth}
%		\input{images/material_compare.pdf_tex}
%		\caption{Sensor measures of human hand with various materials with low $\epsilon_{\text r}$ on top of sensor.}
%	\end{subfigure}
%	\begin{subfigure}{\columnwidth}
%		\centering
%		\def\svgwidth{\columnwidth}
%		\input{images/hand.pdf_tex}
%		\caption{Sensor measures near a non-moving human hand.}
%	\end{subfigure}%
%	\hfill%
%	\begin{subfigure}{\columnwidth}
%		\centering
%		\def\svgwidth{\columnwidth}
%		\input{images/forearm.pdf_tex}
%		\caption{Sensor measures near a non-moving human forearm.}
%	\end{subfigure}
%\end{figure*}

%\begin{figure*}
%	\hfill%
%	\begin{subfigure}{0.3\textwidth}
%		\centering
%		\includegraphics[width=\textwidth, height=125px]{robot_setup_cropped}
%		%\caption{Firts subfigure.}
%		\label{fig:robot_setup}
%	\end{subfigure}%
%	\hfill%
%	\begin{subfigure}{0.33333\textwidth}%
%		\centering
%		\def\svgwidth{\columnwidth}
%		\input{images/setup_diagram.pdf_tex}
%		%\caption{Second subfigure.}
%		\label{fig:setup_diagram}
%	\end{subfigure}%
%	\hfill%
%	\begin{subfigure}{0.3\textwidth}%
%		\centering
%		\includegraphics[width=\textwidth,height=125px]{robot_hand_scan_cropped}
%		%\caption{Second subfigure.}
%		\label{fig:robot_hand_scan}
%	\end{subfigure}
%	\hfill
%	%\vspace{-1.5em}
%	\caption{Experimental setup with capacitive sensor and processing board affixed to the end effector of a Franka Emika 6-DoF robotic arm.}
%	\label{fig:robot_setup_figure}
%\end{figure*}
